CodeAgent: Enhancing Code Generation with Tool-Integrated Agent Systems for Real-World Repo-level Coding Challenges

Large Language Models (LLMs) have shown promise in automated code generation but typically excel only in simpler tasks such as generating standalone code units. Real-world software development, however, often involves complex code repositories (named repo) with complex dependencies and extensive documentation. To fill this gap, our research pivots towards evaluating LLMs in a more realistic setting -- real-world repo-level code generation. We introduce CodeAgentBench, a manually curated benchmark for repo-level code generation. This benchmark comprises five high-quality Python projects, encompassing a total of 101 samples. We assess nine leading LLMs on repo-level tasks and observe a decline in their performance. To tackle this, we present CodeAgent, a novel LLM-based agent framework that employs external tools for effective repo-level code generation. CodeAgent integrates five programming tools, enabling interaction with software artifacts for information retrieval, code symbol navigation, and code testing. We implement four agent strategies to optimize these tools' usage. Our experiments on CodeAgentBench show that CodeAgent enhances LLM performance significantly, with improvements ranging from 18.1\% to 250\%. Further tests on the HumanEval benchmark confirm CodeAgent's adaptability and efficacy across various code generation tasks. Notably, CodeAgent outperforms commercial products like Github Copilot, showcasing superior accuracy and efficiency. These results demonstrate CodeAgent's robust capabilities in code generation, highlighting its potential for real-world repo-level coding challenges.

==> discussion.tex <==
%待明确内容
%数据集时间，涉及数据泄露问题
%



%现有代码生成数据集的缺点，1 简单，独立； 2 输入单一？ 
%不能测评现有模型在真实使用场景上的表现，因此我们提出一个反映真实使用场景的repo-level的数据集。
%增加：验证发现，现有的模型在repo-level上的表现并不好，
%为了提升模型在repo-level数据上的生成能力。我们提出....
%--------
%我们数据集的优势：多domain 优势不明显。
%我们数据集更贴近真实使用场景的表现：1 repo-level 2 多模态输入； 3 多依赖；4 具有运行环境;
%--------
% chapter3 Repo-level Coding Challenges
%table1  Input Information不清晰；可以加个level一列/dependency一列；
%加示例
%--------
%chapter4 Proposed Method
%关于tool，可以想个递进关系/优劣关系 最好不要单纯的罗列 （分门别类？）
%关于agent，可以结合code feature解释为什么用这几个agent，也不是单纯罗列，或者直接写上优缺点，并通过后面的结果论证。
%--------
%Background和 related work可以合并
%数据集feature和优势 写一个就可以了；可以写feature
% （符合代码生成任务的特性）
%放示例 结果



